Sunyaev-Zeldovich Signals from $L^*$ Galaxies: Observations, Analytics, and Simulations

We analyze measurements of the thermal Sunyaev-Zeldovich (tSZ) effect arising in the circumgalactic medium (CGM) of $L^*$ galaxies, reported by Bregman et al. 2022 and Das et al. 2023. In our analysis we use the Faerman et al. 2017 and Faerman et al. 2020 CGM models, a new power-law model (PLM), and the TNG100 simulation. For a given $M_{\rm vir}$, our PLM has four parameters; the fraction, $f_{\rm hCGM}$, of the halo baryon mass in hot CGM gas, the ratio, $\phi_T$, of the actual gas temperature at the virial radius to the virial temperature, and the power-law indicies, $a_{P,{\rm th}}$ and $a_n$ for the thermal electron pressure and the hydrogen nucleon density. The B+22 Compton-$y$ profile implies steep electron pressure slopes ($a_{P,{\rm th}}\simeq 2$). For isothermal conditions the temperature is at least $1.1\times 10^6$ K, with a hot CGM gas mass of up to $3.5\times 10^{11}$ M$_\odot$ for a virial mass of $2.75\times 10^{12}$ M$_\odot$. However, if isothermal the gas must be expanding out of the halos. An isentropic equation of state is favored for which hydrostatic equilibrium is possible. The B+22 and D+23 results are consistent with each other and with recent (0.5-2 keV) CGM X-ray observations by Zhang et al. 2024 of Milky Way mass systems. For $M_{\rm vir}\simeq 3\times 10^{12}$ M$_\odot$, the scaled Compton pressure integrals, $E(z)^{-2/3}Y_{500}/M_{\rm vir,12}^{5/3}$, lie in the narrow range, $2.5\times 10^{-4}$ to $5.0\times 10^{-4}$ kpc$^2$, for all three sets of observations. TNG100 underpredicts the tSZ parameters by factors $\sim 0.5$ dex for the $L^*$ galaxies, suggesting that the feedback strengths and CGM gas losses are overestimated in the simulated halos at these mass scales.

==> tb_FSM_B_TNG_PLM.tex <==
\begin{table*}[]
\centering
\caption{PLM parameters.}

\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
                             & $M_{\rm vir, 12}$ & $f_{\rm hCGM}$ & $\phi_{T}$ & $a_{P,\rm th}$ & $a_n$ & $\phi_T^*$ & \textcolor{red}{$y(0.2) E^{-2} / M_{\rm vir, 12}$} & \textcolor{red}{$Y_{500} E^{-2/3} /  M_{\rm vir, 12}^{5/3}$} \\ \hline
FSM17                        & 1.0     & {\oran{0.76}}       & {\oran{3.05}}     & {\oran{0.78}}       & {\oran{0.72}}  & {\oran{10.64}}      & \textcolor{red}{$2.02 \times 10^{-8}$}                     & \textcolor{red}{$5.12 \times 10^{-4}$}                     \\
FSM20-maximal                      & 1.0     & {\oran{0.59}}       & \textcolor{red}{0.71}       & \textcolor{red}{1.64}       & \textcolor{red}{0.98}  & \textcolor{red}{1.67}       & \textcolor{red}{$0.70 \times 10^{-8}$}                    & \textcolor{red}{$0.99 \times 10^{-4}$}                    \\
FSM20                        & 1.0     & 0.29    &   \textcolor{red}{0.71}       & \textcolor{red}{1.64}       & \textcolor{red}{0.98}  & \textcolor{red}{0.83}       & \textcolor{red}{$0.35 \times 10^{-8}$}                    & \textcolor{red}{$1.98 \times 10^{-4}$}                   \\
% TNG100 (SF) & 1.0     & 0.37       & 0.95       & 2.13       & 1.71  & 0.91       & 1.4                    & 1.3                    \\
TNG100 (SF, $L^*$) & $0.3-3$  & $0.30-0.43$       & $0.81-0.96$       & $1.82-2.28$       & $1.49-1.83$  & $0.57-1.24$       & \textcolor{red}{$(0.35-0.81) \times 10^{-8}$}                    & \textcolor{red}{$(1.05-2.73) \times 10^{-4}$}                    \\
B+22 (isothermal)                  & 2.75     & 0.83          & 1.48          & 2.03       & 2.03     & 2.39       & \textcolor{red}{$1.47 \times 10^{-8}$}                    & \textcolor{red}{$4.55\times10^{-4}$}                    \\
B+22 (isentropic)                   & 2.75     & $0.45 - 0.83$          & $1.48-0.81$          & 2.03       & 1.22     & 2.39       & \textcolor{red}{$(1.46-1.48) \times 10^{-8}$}                    & \textcolor{red}{$(4.53-4.57)\times 10^{-4}$}                    \\
Z+24 (isothermal)                        & 1.4     & 0.51       & 2.56       & 1.26       & 1.26   & 4.54   & \textcolor{red}{$1.18 \times 10^{-8}$}                      & \textcolor{red}{$3.08 \times 10^{-4}$}                    \\ \hline
\end{tabular}
\tablecomments{{\oran{The PLM parameters for FSM17 are for the gas distributions following the formation of the OVI component (see \S~\ref{sec:PLMFSM}).}} The PLM parameters for \citetalias{Bregman2022} are those for which $\eta_{\rm vir}\ge 1$ and hydrostatic equilibrium (HSE) is possible (see \S~\ref{sec:plm-b22}). }
\label{tab:PLM_parameters}
\end{table*}

==> tb_new.tex <==

\renewcommand{\arraystretch}{1.2} % Default value: 1

\begin{table}
\centering
	\caption{Summary of numbers}
	\begin{tabular}{| l || c | c | c |}
	
        \midrule
	model 0 & model 1 & model 2 & model 3 \\
        \midrule
        parameter 1    & $250$ & $283$     & $XX$       \\
        parameter 2    & $0.5$ & $0.3-1.0$ & $0.15-0.5$ \\
        \midrule
	$N_{\rm OVI}~(\cmc)$   & $2.5 \times 10^{14}$ & $2.9 $ & $3.4$ \\
	$XX$                   & $4.5$                &  $4.2$ & $4.9$ \\

    % \midrule
    % Footnotes:
    % \multicolumn{6}{| l |}{(i) In the isentropic model, the CGM extent is a free parameter, and in the fiducial model it is $R_{\rm CGM} = 1.1 R_{\rm vir}.$} \\
    
    \bottomrule
    \end{tabular}
    \vspace{0.5 cm}
  \label{tab:tb_new}
\end{table}


